Concept-based Adversarial Attacks: Tricking Humans and Classifiers Alike

We propose to generate adversarial samples by modifying activations of upper layers encoding semantically meaningful concepts. The original sample is shifted towards a target sample, yielding an adversarial sample, by using the modified activations to reconstruct the original sample. A human might (and possibly should) notice differences between the original and the adversarial sample. Depending on the attacker-provided constraints, an adversarial sample can exhibit subtle differences or appear like a "forged" sample from another class. Our approach and goal are in stark contrast to common attacks involving perturbations of single pixels that are not recognizable by humans. Our approach is relevant in, e.g., multi-stage processing of inputs, where both humans and machines are involved in decision-making because invisible perturbations will not fool a human. Our evaluation focuses on deep neural networks. We also show the transferability of our adversarial examples among networks.

==> related_work.tex <==
\section{Background and Motivation}
\label{sec:related}
Machine Learning (ML) solutions represent a valuable asset for modern tasks~\cite{jordan2015machine}, and the capabilities of ML are further extended by Deep Learning (DL) methods~\cite{lecun2015deep}. However, many efforts have shown that all such methods are vulnerable to \textit{adversarial attacks} (e.g.,~\cite{biggio2013evasion}), giving birth to a new research area commonly referred to `adversarial machine learning'~\cite{biggio2018wild}. We summarize related works in this domain, and then provide the motivation of this paper.

\subsection{Adversarial Attacks}
\label{ssec:background}
Adversarial attacks leverage the so-called `adversarial examples': the principle is to apply a perturbation to an input sample, aiming to induce an incorrect output from the target ML model~\cite{papernot2018sok}. Previous efforts amply showed that adversarial examples can defeat any ML model. For instance, similar attacks have broken both traditional ML models (e.g., SVM~\cite{pierazzi2020intriguing}) as well as DL ones (e.g.,~\cite{su2019one}). Noteworthy is also that adversarial attacks can be successful in diverse domains (and, hence, on different data-types), such as computer vision~\cite{su2019one}, speech analysis~\cite{cisse2017houdini}, or cyber detection~\cite{apruzzese2019addressing}. Even \textit{real} ML systems have been defeated (e.g.,~\cite{liang2016cracking}). 



The major discriminant between adversarial attacks are their \textit{requirements}, which are typically expressed via a \textit{threat model}. Such threat model describes the relationship of the attacker with the targeted system, usually in the form of \textit{goal}, \textit{knowledge}, \textit{capability} and \textit{strategy}~\cite{biggio2018wild}. Common terms associated to such threat models are `white-box' and `black-box'~\cite{papernot2018sok}: the former envision attackers with complete knowledge of the target system, whereas in the latter the attacker knows nothing. Depending on such assumptions, the attacker can opt for different strategies, such as crafting the `perfect' perturbation---e.g., the well-known `Projected Gradient Descent' (PGD) method~\cite{madry2018towards}---or exploit the \textit{transferability} property of adversarial examples~\cite{demontis2019adversarial}. Although all adversarial attacks share the same objective (i.e., compromising the decisions of a ML system), the attacker may have more specific goals: for instance, they can aim at minimizing the perturbations~\cite{su2019one}, reducing the amount of interactions with the target system~\cite{papernot2017practical}, or inducing a `targeted' output~\cite{carlini2018audio}.

Hence, the unique traits of this paper with respect to previous work lie in our assumed threat model---and, specifically, in the \textit{goal} and \textit{strategy} of our attacker. Indeed, we assume that the attacker wants to introduce perturbations that \textit{can be spotted by a human}; to do so, the attacker leverages \textit{high-level concepts} provided by the first layers of deep neural networks\footnote{As such, our proposal is specific of Deep Learning.}. Such methodology is considerably different than those proposed by previous work (e.g.,~\cite{su2019one, moosavi2016deepfool}). 
In particular, our perturbations involve techniques (i.e.,~\cite{sch21cla, van20}) within the \textit{explainable machine learning} domain~\cite{bhatt2020explainable}: some papers use similar techniques to `explain' adversarial attacks (e.g.,~\cite{amich2021explanation}), but no paper uses such techniques to `generate' adversarial samples---to the best of our knowledge.

%% ALTERNATIVE VERSION OF THE SENTENCE ABOVE
% In particular, our perturbations involve techniques (i.e.,~\cite{sch21cla, van20}) within the \textit{explainable machine learning} domain~\cite{bhatt2020explainable}. This is an emerging research area that has recently been linked to adversarial ML, although typically for different purposes: for instance, the authors of~\cite{amich2021explanation} try to `explain' adversarial attacks, whereas we use such techniques to `generate' adversarial examples.











\subsection{Motivation}
\label{ssec:motivation}
Our method aims to craft human-recognizable perturbations by leveraging the ideas in~\cite{sch21cla, van20}, which require accessing and complete knowledge to a trained deep neural network (DNN).
Let us explain why our findings are worthy of being investigated from a security perspective. 
Specifically, we focus on: (i) human-recognizable perturbations; (ii) the requirements to stage the attack; and (iii) additional security benefits.

\textbf{Human-recognizable perturbations.}
Consider the user of an online marketplace who wants to sell an item, and hence uploads some photos of such item. Many online marketplaces already rely on DL to estimate the value of an object from its images~\cite{var18}.
The seller (i.e., the attacker) may want to trick the DL model to output higher prices via some perturbations; however, doing this without significantly enhancing the photos would discourage any buyer from purchasing the car (i.e., the high price would not be justified). Hence, minimal perturbations (e.g.~\cite{su2019one}) would have no tangible benefit for the attacker, who must ensure that the alterations result in a different perception of the sample by the human\footnote{To prevent the adversarial example from falling in a different class, we apply some constraints on the magnitude of the perturbations.}.

\textbf{Requirements.} 
Our method requires complete knowledge of a DNN, which can be associated to `white-box' attackers. We observe that, in some domains, our assumptions are viable: for instance, many DL systems are trained on the ImageNet dataset~\cite{kornblith2019better}, which is publicly available~\cite{deng2009imagenet}. In these settings, even a `black-box' attacker can be successful, because they can create a surrogate DL model and transfer the successful adversarial examples to the target DL model~\cite{demontis2019adversarial}. We acknowledge that, in some domains, our attacks may be difficult to stage: for instance, ML security systems are well-protected~\cite{apruzzese2021modeling}; however, it would make little sense to aim for `human-recognizable' perturbations against similar systems.

\textbf{Additional Benefits.}
From a security standpoint, we observe that any \textit{offense} can be turned into a \textit{defense}. In our case this can be done via the well-known \textit{adversarial training} technique~\cite{ganin2016domain, shafahi2019adversarial}: indeed, many papers propose to first attack a ML model, and then use the successful attacks to harden such ML model (e.g.,~\cite{apruzzese2020deep}). Such property allows our method to be applicable---as a defense---also in scenarios where the `white-box' assumptions are unfeasible for an attacker (i.e., the defender has obviously full control of their own ML system).
 
In our paper, we assume a computer vision task, but the underlying principles of our method are agnostic of the data-type, and hence applicable also to DL applications for other domains (e.g., malware detection~\cite{kolosnjaji2018adversarial})
